Solving Schr\"{o}dinger bridge problem via continuous normalizing flow

The Schr\"{o}dinger Bridge Problem (SBP), which can be understood as an entropy-regularized optimal transport, seeks to compute stochastic dynamic mappings connecting two given distributions. SBP has shown significant theoretical importance and broad practical potential, with applications spanning a wide range of interdisciplinary fields. While theoretical aspects of the SBP are well-understood, practical computational solutions for general cases have remained challenging. This work introduces a computational framework that leverages continuous normalizing flows and score matching methods to approximate the drift in the dynamic formulation of the SBP. The learned drift term can be used for building generative models, opening new possibilities for applications in probability flow-based methods. We also provide a rigorous $\Gamma-$convergence analysis for our algorithm, demonstrating that the neuron network solutions converge to the theoretical ones as the regularization parameter tends to infinity. Lastly, we validate our algorithm through numerical experiments on fundamental cases.

==> sch2ot.tex <==

By adopting the same approach, we can also prove that the Schr\"{o}dinger Bridge Problem $\Gamma-$converges to an optimal transport problem as the diffusion coefficient $\sigma\to 0$. The OT problem can be stated as

\begin{equation}\label{eq:OT}
\begin{array}{ll}
\min\limits_{\rho, m} & \int_{0}^{1} \int_{\mathbb{R}^d} \frac{|m|^2}{2\rho} dx dt, \\
\text { s.t. } &\partial_{t} \rho +\nabla \cdot m=0 ,\\
&\rho(x,0)=\rho_{0}(x), \rho(x, 1)=\rho_1(x).
\end{array}
\end{equation}

and the Schr\"odinger Bridge Problem

\begin{equation}\label{eq:Schb}
\begin{array}{ll}
\min\limits_{\rho, m} & \int_{0}^{1} \int_{\mathbb{R}^d} \frac{|m|^2}{2\rho} dx dt, \\
\text { s.t. } &\partial_{t} \rho +\nabla \cdot m= \sigma^2\Delta\rho,\\
&\rho(x,0)=\rho_{0}(x), \rho(x, 1)=\rho_1(x).
\end{array}
\end{equation}

Let 
\begin{multline}
E_\sigma=\left\{(\rho,m)\in X:-\int_0^1(\int_\Omega(\partial_t\phi)\rho(dx)+\nabla\phi\cdot m(dx))\,dt - \int_\Omega\phi(x,0)\rho_0(dx)\right.\\
\left.+\int_\Omega\phi(x,1)\rho_1(dx)=\sigma^2\int_0^1\int_\Omega\Delta\phi\cdot\rho(dx)\,dt, \forall\phi\in C_b^1(\Omega; [0,1]), m\ll\rho\right\}, 
\end{multline}
and
\begin{multline}
E_\sigma=\left\{(\rho,m)\in X:-\int_0^1(\int_\Omega(\partial_t\phi)\rho(dx)+\nabla\phi\cdot m(dx))\,dt - \int_\Omega\phi(x,0)\rho_0(dx)\right.\\
\left.+\int_\Omega\phi(x,1)\rho_1(dx)=0, \forall\phi\in C_b^1(\Omega; [0,1]), m\ll\rho\right\}, 
\end{multline}
then the solutions to \eqref{eq:OT} and \eqref{eq:Schb} is the minimizers of functionals
\begin{equation}
\begin{aligned}
F_\sigma(\rho, m)&=\int_{0}^{1} \mathscr{B}_2(\rho_t, m_t)\,dt +\chi_{E_\sigma}^{+\infty},\\
F_(\rho, m)&=\int_{0}^{1} \mathscr{B}_2(\rho_t, m_t)\,dt+ \chi_{E}^{+\infty}
\end{aligned}
\end{equation}
respetively.

So we only need to prove that $\chi_{E_\sigma}^{+\infty}$ $\Gamma-$convergence to $\chi_{E}^{+\infty}$, then we can get the minimizers of $F_\sigma$ have a subsequence converges to the minimizers of $F$. Here we use the method borrowed from \cite{xiong_convergence_2024}.

The following lemma gives a sufficient condition of a sequence of indicator functions to be $\Gamma-$convergence.
\begin{lemma}
Suppose $\{E_n\}$ is a sequence of sets in space $X\times Y$. If there exists a set $E_\infty\subset X\times Y$ that satisfies two conditions,
\begin{itemize}
    \item if $x^n\to x$, $y^n\to y$ and $(x^n, y^n)\in E_n$ for infinitely many $n$, then $(x,y)\in E_\infty$.
    \item if $(x,y)\in E_\infty$ and $x^n\to x$, then there exists $y^n\to y$ such that $(x^n, y^n)\in E_n$ for $n$ large enough,
\end{itemize}
then $\chi_{E_n}^{+\infty}$ $\Gamma-$converges to $\chi_{E_\infty}^{+\infty}$.
\end{lemma}

Now consider a sequence of $(\rho^\sigma, m^\sigma)\to(\rho,m)$, $(\rho^\sigma, m^\sigma)\in E_\sigma$, we have
\begin{multline}
-\int_0^1(\int_\Omega(\partial_t\phi)\rho^\sigma(dx)+\nabla\phi\cdot m^\sigma(dx))\,dt - \int_\Omega\phi(x,0)\rho_0(dx)+\int_\Omega\phi(x,1)\rho_1(dx)\\
=\sigma^2\int_0^1\int_\Omega\Delta\phi\cdot\rho^\sigma(dx)\,dt, \forall\phi\in C_b^1(\Omega; [0,1]).
\end{multline}
Let $\sigma\to\infty$ then
\begin{multline}
-\int_0^1(\int_\Omega(\partial_t\phi)\rho(dx)+\nabla\phi\cdot m(dx))\,dt - \int_\Omega\phi(x,0)\rho_0(dx)+\int_\Omega\phi(x,1)\rho_1(dx)\\
=0, \forall\phi\in C_b^1(\Omega; [0,1]),
\end{multline}
namely $(\rho,m)\in E$.

We then consider $(\rho, m)\in E$ and $\rho^\sigma\to\rho$. We want to find $m^\sigma$ such that
\begin{multline}
-\int_0^1(\int_\Omega(\partial_t\phi)\rho^\sigma(dx)+\nabla\phi\cdot m^\sigma(dx))\,dt - \int_\Omega\phi(x,0)\rho_0(dx)+\int_\Omega\phi(x,1)\rho_1(dx)\\
=\sigma^2\int_0^1\int_\Omega\Delta\phi\cdot\rho^\sigma(dx)\,dt, \forall\phi\in C_b^1(\Omega; [0,1]).
\end{multline}

By Helmholtz decomposition, we obtain
$m=-\nabla\Phi + h$, where $\nabla\cdot h=0$. Let $\Phi^\sigma$ be such that
\begin{multline}
-\int_0^1(\int_\Omega(\partial_t\phi)\rho^\sigma(dx)+\nabla\phi\cdot \nabla\Phi^\sigma(dx))\,dt - \int_\Omega\phi(x,0)\rho_0(dx)+\int_\Omega\phi(x,1)\rho_1(dx)\\
=\sigma^2\int_0^1\int_\Omega\Delta\phi\cdot\rho^\sigma(dx)\,dt, \forall\phi\in C_b^1(\Omega; [0,1]).
\end{multline}

$\Phi^\sigma$ exists since it is the solution of Poisson equation

\begin{equation}
-\Delta \Phi^\sigma = \partial_t\rho^\sigma + \sigma^2\Delta \rho^\sigma.
\end{equation}

We have
\begin{equation}
-\Delta (\Phi^\sigma-\Phi) = \partial_t(\rho^\sigma-\rho)+\sigma^2\Delta(\rho^\sigma-\rho),
\end{equation}
hence $\Phi^\sigma\to\Phi$ as $\sigma\to 0$.

Let $m^\sigma = -\nabla\Phi^\sigma + h$, then $(\rho^\sigma, m^\sigma)\in E_\sigma$ and $m^\sigma\to m$. Hence $F_\sigma$ $Gamma-$converges to $F$. With the lower semi-continuity of $F_\sigma$ and $F$, minimizers of $F_\sigma$ and $F$ exist, and for any minimizer $(\rho^\sigma, m^\sigma)$ if $F_\sigma$, there exists a subsequence $(\rho^{\sigma_k}, m^{\sigma_k})$ converging to the minimizer $(\rho, m)$ of $F$.
